OTTers: One-turn Topic Transitions for Open-Domain Dialogue

Mixed initiative in open-domain dialogue requires a system to pro-actively introduce new topics. The one-turn topic transition task explores how a system connects two topics in a cooperative and coherent manner. The goal of the task is to generate a "bridging" utterance connecting the new topic to the topic of the previous conversation turn. We are especially interested in commonsense explanations of how a new topic relates to what has been mentioned before. We first collect a new dataset of human one-turn topic transitions, which we call OTTers. We then explore different strategies used by humans when asked to complete such a task, and notice that the use of a bridging utterance to connect the two topics is the approach used the most. We finally show how existing state-of-the-art text generation models can be adapted to this task and examine the performance of these baselines on different splits of the OTTers data.

==> OTTers dataset/table_corpus_properties.tex <==
    \begin{tabular}{|l|r|}
        % All numbers current as of 2021-02-01 at 10:18
        \hline
        Property  & \textbf{\dataset} \\
        \hline
        \textbf{TTR}       & $5085$ / $70935$\\
        \hline
        \textbf{ent.\ TTR}  &  $3984$ / $17054$\\
        \hline
        \textbf{turn length}  &  $2$-$68$ \\
        ---: mean    & $16.4$\\
        ---: mode    &  $9$\\
        \hline
        \textbf{sent.s/turn}  &  $1$-$7$\\
        ---: mean    &  $1.3$\\ 
        ---: mode    &  $1$\\
        \hline
        \textbf{KG path}      &  $1$-$14$\\
        ---: mean    &   $6.1$\\
        ---: mode    &   $5$\\
        \hline
    \end{tabular}    
% \begin{tabular}{l|r|r}
%         % All numbers current as of 2021-02-01 at 10:18
%         Property & \alphanlg & \dataset \\
%         \hline
%         TTR        & 18340 / 688214 & 5085 / 70935\\
%         % ---: train & 116k   / 1.5M & \\
%         % ---: dev   &  21k   / 222k & \\
%         % ---: test  &  37.7k / 440k & \\
%         \hline
%         ent.\ TTR  &  22317 / 243871 & 3984 / 17054\\
%         % ---: train &  & \\
%         % ---: dev   &  & \\
%         % ---: test  &  & \\
%         \hline
%         turn length  & &  \\
%         ---: min-max & 4-36 &  2-68\\
%         ---: mean    & 9.6  & 16.4\\
%         ---: mode    & 8    &  9\\
%         \hline
%         sent.s/turn  & & \\
%         ---: min-max & 1-4 & 1-7\\
%         ---: mean    & 1.0 & 1.3\\ 
%         ---: mode    & 1   & 1\\
%         \hline
%         KG path      & &  \\
%         ---: min-max & 1-14 & 1-14\\
%         ---: mean    & 5.6  &  6.1\\
%         ---: mode    & 1    &  5\\
%     \end{tabular}

==> OTTers dataset/table_example_outputs.tex <==

\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|p{0.7cm}@{~}|rp{4.6cm}|}
\hline
& Topic A: & I like babies.\\
Ex. 1&\dataset & I make babies laugh.\\
&Topic B: & I enjoy making other people laugh.\\
\hline
&vGPT2:   & I like other people making babies.\\
&\alphanlg: & I decided to give birth to a baby.\\
&\alphanlg{}ft: & I like to make babies laugh when I'm not working.\\
\hline
\hline
&Topic A: & I love those sleek Italian cars.\\
Ex. 2&\dataset & I wish I was as sleek as those cars.\\
&Topic B: & I am in good shape.\\
\hline
&vGPT2:   & I love it. I love it.\\
&\alphanlg: & I bought a new car.\\
&\alphanlg{}ft: & I like the look of Italian cars.\\
\hline
\hline
&Topic A: & I have prior agriculture experience.\\
Ex. 3&\dataset & My parents were farmers.\\
&Topic B: & I am a mom.\\
\hline
&vGPT2:   & a lot of cooking. I am a lot of cooking.\\
&\alphanlg: & My mom taught me how to grow vegetables.\\
&\alphanlg{}ft: & I have been a farmer for many years.\\
\hline
\hline
&Topic A: & I make blogs.\\
Ex. 4&\dataset & Do you know of any blogs that are on the subject of large families with babies?\\
&Topic B: & I have a large family with babies.\\
\hline
&vGPT2:   & family.\\
&\alphanlg: & I have a lot of babies.\\
&\alphanlg{}ft: & I have a large family.\\
% \hline
% \hline
% Topic A: & \\
% \dataset & \\
% Topic B: & \\
% \hline
% vGPT2:   & \\
% \alphanlg: & \\
% \alphanlg{}ft: & \\
% \hline
% \hline
% Topic A: & \\
% \dataset & \\
% Topic B: & \\
% \hline
% vGPT2:   & \\
% \alphanlg: & \\
% \alphanlg{}ft: & \\
% \hline
% \hline
% Topic A: & \\
% \dataset & \\
% Topic B: & \\
% \hline
% vGPT2:   & \\
% \alphanlg: & \\
% \alphanlg{}ft: & \\
% \hline
% \hline
% Topic A: & \\
% \dataset & \\
% Topic B: & \\
% \hline
% vGPT2:   & \\
% \alphanlg: & \\
% \alphanlg{}ft: & \\
% \hline
% \hline
% Topic A: & \\
% \dataset & \\
% Topic B: & \\
% \hline
% vGPT2:   & \\
% \alphanlg: & \\
% \alphanlg{}ft: & \\

% \begin{tabular}[c]{@{}p{3cm}@{}}\footnotesize{Sent A: Everyday, I get around the city in my big midnight colored vehicle.}\\ \footnotesize{Sent B: I hate throwing out plastic.}\end{tabular} & \footnotesize{my car.} & \footnotesize{I decided to paint my car red.}   & \footnotesize{I like to drive my car in the dark.} & \footnotesize{I don't have a car because I don't want to waste energy. I hate wasting plastic too.}      \\
% \hline
% \begin{tabular}[c]{@{}p{3cm}@{}}\footnotesize{Sent A: My parents had many children.}\\ \footnotesize{Sent B: I am a realtor as well as a waitress.}\end{tabular}                              & \footnotesize{as well as well as well.}    & \footnotesize{My parents divorced when I was a teenager.} & \footnotesize{My parents had many children as well.}    & \footnotesize{My mom raised me by herself while working at a restaurant.}    \\
% \hline
% \begin{tabular}[c]{@{}p{3cm}@{}}\footnotesize{Sent A: Role playing is my favorite hobby.}\\ \footnotesize{Sent B: I can memorize lines.}\end{tabular}                     & \footnotesize{my favorite movies. I like to memorize my favorite movies.} & \footnotesize{I learned a lot of new lines.}  & \footnotesize{My favorite hobby is memorizing lines.}  & \footnotesize{Yes, I like to role play also. I am pretty good at it, too, because I can memorize lines.} \\
% \hline
% \begin{tabular}[c]{@{}p{3cm}@{}}\footnotesize{Sent A: I have some problems with pronunciation.}\\ \footnotesize{Sent B: I have been known to tickle the ivories.}\end{tabular} & \footnotesize{I have been a lot of my hair.} & \footnotesize{I tried to learn the pronunciation of ivy.} & \footnotesize{I don't know how to pronounce the word ivy.}  & \footnotesize{I used to have problems with stuttering, and then buried myself in music.}     \\
% \hline
% \begin{tabular}[c]{@{}p{3cm}@{}}\footnotesize{Sent A: I enjoy making things artistically.}\\ \footnotesize{Sent B: Being a determined lady gets me far in life.}\end{tabular} & \footnotesize{being a woman.}                 & \footnotesize{I decided to make my own.} & \footnotesize{I like to make things myself.}  & \footnotesize{I made a 40 foot sculpture once.} \\
\hline
\end{tabular}
\caption{Representative outputs from each model.}
\label{tab:output_exs}
\end{table}
